SQUID: Faster Analytics via Sampled Quantile Estimation

Streaming algorithms are fundamental in the analysis of large and online datasets. A key component of many such analytic tasks is $q$-MAX, which finds the largest $q$ values in a number stream. Modern approaches attain a constant runtime by removing small items in bulk and retaining the largest $q$ items at all times. Yet, these approaches are bottlenecked by an expensive quantile calculation. This work introduces a quantile-sampling approach called SQUID and shows its benefits in multiple analytic tasks. Using this approach, we design a novel weighted heavy hitters data structure that is faster and more accurate than the existing alternatives. We also show SQUID's practicality for improving network-assisted caching systems with a hardware-based cache prototype that uses SQUID to implement the cache policy. The challenge here is that the switch's dataplane does not allow the general computation required to implement many cache policies, while its CPU is orders of magnitude slower. We overcome this issue by passing just SQUID's samples to the CPU, thus bridging this gap. In software implementations, we show that our method is up to 6.6x faster than the state-of-the-art alternatives when using real workloads. For switch-based caching, SQUID enables a wide spectrum of data-plane-based caching policies and achieves higher hit ratios than the state-of-the-art P4LRU.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

PDFLATEX ?= pdflatex
TEX = $(wildcard *.tex)

pdf: paper.pdf

clean:
	$(RM) *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

%.pdf: $(TEX) $(wildcard *.bib)
	$(PDFLATEX) $*
	-bibtex $*
	if [ -e $*.toc ] ; then $(PDFLATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	$(PDFLATEX) $*


toc: $(wildcard *.tex)
	@egrep -h "\\\((sub)*section|chapter)" $+ | egrep -v "^%" | \
                sed -e 's/\\chapter//;                          \
                s/\\section/    /;                              \
                s/\\subsection/         /;                      \
                s/\\subsubsection/                      /;      \
                s/\\.*{//g;s/[{}]//g' > $@


==> conclusion_old.tex <==
\section{Conclusion}
Our work combines statistical insights with applied algorithm design. We observe that finding an exact quantile is a performance bottlenecks in~\cite{qMax}, and thus we circumvent this bottleneck by finding approximate quantiles by employing a sampling based method.  We show that our method is considerably faster when $q$ is large enough. We argue that large $q$ values are desired since DRAM memory is bountiful, and measurement algorithms are wise to leverage that resource for better accuracy. Then we demonstrated a varying throughput improvement accross measurement applications levraging the \qMAX pattern.  Intuitively, since we only improve a specific operation within these algorithms, the benefits vary depanding how dominant that operation is. Here, the largest improvement is to network-wide heavy hitters~\cite{NetworkWideANCS}, and the smallest is for priority based aggregation (PBA)~\cite{PrioritySampling} the reason for such variability is the portion of time consumed by the \qMAX interface in each of these problems. Indeed, PBA also perform division operations per update are its performance bottleneck. 

We continued our algorithmic and focused only on the single device heavy hitter problem. Here we observed current algorithms~\cite{IMSUM,DIMSUM} and noticed that the performance bottleneck lies in performing a maintenance operation that periodically deletes non-heavy hitter flows.

\looseness=-1
We designed algorithms to solve this problem, namely we designed a  Monte Carlo \qMAX{} version where the algorithm may fail with a low probability.  Such a relaxation allows us to avoid verifying that the probabilistic solution to the \qMAX{} problem is correct. We found intelligent ways to divide this error budget across a measurement of unknown length, and proved that our method is asymptotically optimal \mbox{with a leading constant of two.  }

\looseness=-1
Next, we presented a lazy deletion technique to avoid making a pass to delete non-heavy hitter items. Such a technique when coupled with our Monte Carlo algorithm that requires no pass for verification eliminates the need to make a linear pass within maintenance operations. We then performed an extensive evaluation using real Internet traces. Our evaluation shows benefits in speed due to handling the bottlenecks, and in accuracy since our lazy-deletion \mbox{method retains more information.}
